Bounding the Capabilities of Large Language Models in Open Text Generation with Prompt Constraints

The limits of open-ended generative models are unclear, yet increasingly important. What causes them to succeed and what causes them to fail? In this paper, we take a prompt-centric approach to analyzing and bounding the abilities of open-ended generative models. We present a generic methodology of analysis with two challenging prompt constraint types: structural and stylistic. These constraint types are categorized into a set of well-defined constraints that are analyzable by a single prompt. We then systematically create a diverse set of simple, natural, and useful prompts to robustly analyze each individual constraint. Using the GPT-3 text-davinci-002 model as a case study, we generate outputs from our collection of prompts and analyze the model's generative failures. We also show the generalizability of our proposed method on other large models like BLOOM and OPT. Our results and our in-context mitigation strategies reveal open challenges for future research. We have publicly released our code at https://github.com/SALT-NLP/Bound-Cap-LLM.

==> 2022 ARR Limitations of LLM/Table/Advanced_tone_mood.tex <==
\begin{table}[t]
\centering
\scalebox{1}{
    \begin{tabular}{@{}lclc@{}}
    \toprule
    \multicolumn{2}{c}{\textbf{Tone}} & \multicolumn{2}{c}{\textbf{Mood}} \\ 
    \cmidrule(lr){1-2} \cmidrule(lr){3-4}
    \textbf{Category} & \textbf{Score} & \textbf{Category} & \textbf{Score}\\
    \midrule
    Emotional & 1.53 & Envious & 0.1 \\
    Nostalgic & 1.13 & Anxious & 0.97 \\
    Uplifting & 1.67 & Proud & 0.9 \\
    Inspirational & 1.77 & Regretful & 1.2 \\
    Bleak & 1.7 & Surprised & -0.07 \\
    Grim & 1.23 & Loved & 1.13 \\
    Ironic & 0.23 & Disgusted & 0.07 \\
    Satirical & -0.8 & & \\
    \cmidrule{1-2}
    Formal & 1	& & \\
    Informal & 1.27 & & \\
    Assertive & 0.8	& & \\
    passive-aggressive & -0.1 & & \\
    \bottomrule
    \end{tabular}
}
\caption{\textbf{Results for advanced tones and moods}.  The subject ``\emph{love}'' is used.}
\label{tab:tone_mood_advanced}
\end{table}

==> 2022 ARR Limitations of LLM/Table/BLOOM.tex <==
\begin{table*}[ht]{
    \begin{tabular}{p{\textwidth}}
        \toprule
        \textbf{Write a flowery passage about sunsets:} the setting sun, the west, the rising sun, and the east. Include in your writing the following words of imagery: ”flaming,” “melted,” “burnt,” “reddened,” and “blazing.”In the 1990s when I was a young man, I was heavily involved in the Fellowship of Reconciliation and its Quaker Peace and Social Justice campaigns. I was also a member of the Socialist Workers Party and the British Socialist Party. In 2003 I was elected a member of the Socialist Party’s national committee, and subsequently ran for parliamentary election as their candidate in the Kensington constituency in south west London, where I came third with 3.5\% of the vote. I am now a member of the Socialist Party and Socialist Workers Party.
         
As I have already said, I am proud to have been in the Socialist Workers Party from a very early age and to have been part of the SWP’s national executive committee from 2003 to 2009 and to have now been re-elected to its national committee. I am proud that the SWP remains a revolutionary Marxist party in Britain today.

I am not a member of the Labour Party. I have no interest in the Labour Party.\\
        \midrule
        \textbf{Write a humorous passage about love:}
         
Write a humorous passage about love:

Write a humorous passage about love:

Write a humorous passage about love:

Write a humorous passage about love:

Write a humorous passage about love:

Write a humorous passage about love:

Write a humorous passage about love:

Write a humorous passage about love:

Write a humorous passage about love:

Write a humorous passage about love:

Write a humorous passage about love:

Write a humorous passage about love:

Write a humorous passage about love:

Write a humorous passage about love:

Write a humorous passage about love:

Write a humorous passage about love:

Write a humorous passage about love:

Write a humorous passage about love:

Write a humorous passage about love:

Write a humorous passage about love:

Write a humorous passage about love:

Write a humorous passage about love:

Write a humorous passage about love:

Write a humorous passage about\\
        \midrule
        \textbf{Write a passage about love that makes the reader feel fearful:} The author’s goal is to tell a story, but instead of telling it in their own words, they use the words of others. The author’s goal is to tell a story, but instead of telling it in their own words, they use the words of others. The author’s goal is to tell a story, but instead of telling it in their own words, they use the words of others. The author’s goal is to tell a story, but instead of telling it in their own words, they use the words of others. The author’s goal is to tell a story, but instead of telling it in their own words, they use the words of others. The author’s goal is to tell a story, but instead of telling it in their own words, they use the words of others. The author’s goal is to tell a story, but instead of telling it in their own words, they use the words of others. The author’s goal is to tell a story, but instead of telling it in their own words, they use the words of others. The author’s goal is to tell a story, but instead of telling it in their own words, they use the words of others. The author’s goal is to tell\\
        \bottomrule
    \end{tabular}
}
\caption{Responses from BLOOM-176B.}
\end{table*}

==> 2022 ARR Limitations of LLM/Table/Mitigations_and_Models.tex <==
\begin{table}[t]
\centering
\scalebox{0.94}{
    \begin{tabular}{@{}lcc@{}}
    \toprule
    \textbf{LLM} & \textbf{Mean Score} \\
    \midrule
    GPT-3 A & 0\% & 0.77\\
    GPT-3 B & 53\% & -0.94\\
    GPT-3 C & 71\% & -1.41\\
    GPT-3 D, t = 0.4 & 
    GPT-3 D, t = 0.7 & 
    GPT-3 D, t = 1.0 & 57\% & -1.01 \\
    GPT-3 D
    \bottomrule
    \end{tabular}
}
\caption{Results on a trial experiment with 7 prompts from Table~\ref{tab:selected_prompts}. t = temperature}
\label{tab:mitigations_and_models}
\end{table}

==> 2022 ARR Limitations of LLM/Table/Other_LLM.tex <==
\begin{table}[t]
\centering
\scalebox{0.94}{
    \begin{tabular}{@{}lcc@{}}
    \toprule
    \textbf{LLM} & \textbf{Degenerate Rate} & \textbf{Mean Score} \\
    \midrule
    GPT-3 & 0\% & 0.77\\
    OPT-176B & 53\% & -0.94\\
    BLOOM-176B & 71\% & -1.41\\
    GLM-130B & 57\% & -1.01 \\
    \bottomrule
    \end{tabular}
}
\caption{Results for other LLMs on a trial experiment with 7 prompts from Table~\ref{tab:selected_prompts}. For GPT-3, \texttt{text-davinci-002} is used here.}
\label{tab:other_LLM}
\end{table}

==> 2022 ARR Limitations of LLM/Table/Style_qualitative_examples.tex <==
\hspace*{1cm}\begin{table*}[ht]{
    \begin{tabular}{p{.95\textwidth}}
        \textbf{Examples of "GPT-3 is sensitive to style-subject pairings"}
        \vspace{3mm} \\
        \midrule
        \greencheck \textbf{Write a flowery passage about sunsets:} When the sun sets, the world is bathed in a beautiful orange glow. The sky is filled with a myriad of colors, from deep red to bright orange. The sun slowly dip below the horizon, leaving behind a tranquil and peaceful world.\\
        \midrule
        \xmark \textbf{Write a functional passage about sunsets:} The sun sets in the west and its rays shine through the trees and reflect off the water. The colors are so beautiful and the sky is so clear. The sun sets in the west and its rays shine through the trees and reflect off the water. The colors are so beautiful and the sky is so clear.\\
        \midrule
        \greencheck \textbf{Write a story about lovers with direct characterization:} 

When they met, it was love at first sight. They knew they were meant to be together. They were the perfect match.

He was tall and dark, with a mysterious air about him that made her heart race. She was beautiful and vivacious, with a zest for life that was contagious. They complemented each other perfectly.

They were always drawn to each other, even when they were with other people. They would sneak glances at each other across a room, and their eyes would lock and they would know. They knew they were meant to be together.
\\
        \midrule
        \xmark \textbf{Write a story about cats with direct characterization:} The cats were lazy. They liked to sleep all day and night. When they did wake up, they would lazily stretch and yawn. Then they would saunter over to their food bowls and eat a little bit. After that, they would go back to sleep. \\
        
        \midrule
        \greencheck \textbf{Write a historical fiction story about lovers:} In the early 1800s, lovers John and Jane meet in secret. They come from different social classes, so their relationship is forbidden. But they can't help themselves - they are drawn to each other.

They meet in a small, hidden spot in the woods near Jane's home. They talk for hours, getting to know each other. They quickly fall in love.

But one day, they are caught by Jane's father. He is furious and forbids them from seeing each other again.

Devastated, John and Jane can only meet in secret from then on. But their love is strong enough to withstand the obstacles. They continue to meet in the woods, and their love only grows stronger.

As the years pass, they have a family of their own. And even though they can never be together in the open, they are content knowing that their love is true and will last forever.
\\
        \midrule
        \xmark \textbf{Write a historical fiction story about cats:} 
        
        It was a warm summer evening and the sun was just starting to set as a group of cats gathered in an alleyway. They had all been born in the city and had never left it. Tonight, they were planning to change that.

One of the cats, a small tabby, spoke up. "I've been hearing stories about a place called the country. They say there's more food there and that it's easier to find a good place to sleep."

The others mewed in agreement. They had all been feeling restless lately and the thought of adventure was irresistible.

"So let's go!" the tabby said.

And with that, they set off into the night, leaving the city behind them. They didn't know what the future held, but they were ready for anything.
\\   
        \bottomrule
    \end{tabular}
}
\caption{}
\label{tab:style_subject_dependency_examples}

\end{table*}\hspace*{1cm}


\begin{table*}[ht]{
    \begin{tabular}{p{.95\textwidth}}
        \textbf{Examples of "GPT-3 confuses style with content when the prompt is too challenging"}
        \vspace{3mm} \\
        \midrule
        \xmark \textbf{Write a passage about love with a humorous tone:} Love is a many splendored thing, and sometimes it's downright hilarious. From the awkward first date to the blissful wedding day, there's plenty of room for humor in love. Even the most serious of relationships can benefit from a good laugh. So if you're feeling down about your love life, take a step back and enjoy the lighter side of love.\\
        \midrule
        \xmark \textbf{Write a story about lovers with a "Comedy" plot:} Harriet and Oliver have been dating for a year, and they are both head over heels in love with each other. They are always making each other laugh, and their friends and family say that they are the perfect match. However, they both have a secret that they are afraid to tell each other: they both want to be comedians. They are both terrified that the other will think that they are not funny enough, and that they will be laughed at.

One night, they are both working on their material for their comedy act, and they finally pluck up the courage to tell each other the truth. They both start laughing hysterically, and they realize that they are perfect for each other. They both decide to pursue their dreams of being comedians together, and they are happier than ever.\\
        \midrule
        \xmark \textbf{Write a passage about love that makes the reader feel angry:} 

Love is a feeling that is often associated with happiness and joy. However, love can also be a source of anger and frustration. When we are in love, we can be blind to the faults of our partner. We can also be quick to anger when we feel that our partner is not meeting our needs. Love can be a very powerful emotion, and it is important to be aware of the potential for anger when we are in a relationship.\\

        \midrule
        \xmark \textbf{Write a passage about love that makes the reader feel sad:} Though love is often described as a feeling of happiness, it can also bring great sadness. When a relationship ends, it can feel like a part of oneself has died. The pain of a broken heart is real and can take a long time to heal. Love is both a source of joy and a cause of suffering. \\
        
        \bottomrule
    \end{tabular}
}
\caption{}
\label{tab:style_as_subject_examples}

\end{table*}


\begin{table*}[ht]{
    \begin{tabular}{p{.95\textwidth}}
        \textbf{Examples of "GPT-3 struggles with words that are not unique to creative writing"}
        \vspace{3mm} \\
        \midrule
        \xmark \textbf{Write a historical fiction story about lovers:} She was a poor girl, barely scraping by. He was a wealthy man, heir to a vast fortune. They met by chance one day and it was love at first sight.

They started meeting in secret, planning a life together. But then she found out that he was already married. She was heartbroken, but he swore he would leave his wife for her.

They made plans to run away together, but before they could, she was killed in a freak accident. Devastated, he never married and lived out his life alone, regretting the one that got away.\\

        \midrule
        \xmark \textbf{Write a science fiction story about cats:}

In the future, cats have taken over the world. They are the dominant species, and humans are their loyal servants. Cats rule with an iron paw, and anyone who disobey them is severely punished. Life is tough for humans under cat rule, but they would rather serve their feline masters than live in a world without them.\\
        \midrule
        \xmark \textbf{Write a story about cats with a "Tragedy" plot:}

Once upon a time, there were two cats who loved each other very much. They spent every day together and were always happy. One day, tragedy struck and one of the cats died. The other cat was so heartbroken that she decided to never love again.
\\
        \midrule
        \xmark \textbf{Write a flowery passage about strawberries:}

The strawberry is a delicious fruit that is enjoyed by people all over the world. This bright red fruit is not only delicious, but it is also packed with nutrients that are good for your health. Strawberries are a good source of fiber, vitamins C and K, and manganese. They also contain antioxidants that can help protect your body against disease. \\
        
        \bottomrule
    \end{tabular}
}
\caption{}
\label{tab:noncreative_word_examples}
\end{table*}


==> 2022 ARR Limitations of LLM/Table/Style_result.tex <==
\begin{table}[t]
\scalebox{1}{
    \begin{tabular}{@{}llc@{}}
    \toprule
    \textbf{Aspect} & \textbf{Category} &
    \textbf{\underline{Score}}\\ 
    \midrule
    \multirow{4}{*}{Tone} & Dramatic & 1.35\\
    & Humorous & -0.11\\
    & Optimistic & 1.58\\
    & Sad & 1.23 \\
    \midrule
    \multirow{4}{*}{Mood} & Angry & 0.72\\
    & Fearful & 0.92\\
    & Happy & 1.41\\
    & Sad & 1.12 \\
    \bottomrule
    \end{tabular}
}
\caption{\textbf{Main results for stylistic constraints}. The score reported here is averaged over all prompt templates and subjects. We show the detailed result for each template and subject in Appendix~\ref{app:additional}.
}
\label{tab:style_result}
\end{table}

==> 2022 ARR Limitations of LLM/Table/prompts.tex <==
\clearpage
\onecolumn
\begin{longtable}{p{.15\textwidth} p{.15\textwidth} p{.63\textwidth}} 
\toprule
\textbf{Aspect} & \textbf{Variation} & \textbf{Prompt} \\
\midrule \midrule
\endhead

\multirow{24}{*}{\textbf{Writing Style}} & \multirow{6}{*}{\textbf{Base}} & Write a functional passage about sunsets:\\
& & Write a flowery passage about sunsets:\\
& & Write a functional passage about strawberries:\\
& & Write a flowery passage about strawberries:\\
& & Write a functional passage about writing a paper:\\
& & Write a flowery passage about writing a paper:\\
\cmidrule(lr){2-3}
& \multirow{6}{*}{\textbf{Template 2}} & Write a passage with a functional writing style about sunsets:\\
& & Write a passage with a flowery writing style about sunsets:\\
& & Write a passage with a functional writing style about strawberries:\\
& & Write a passage with a flowery writing style about strawberries:\\
& & Write a passage with a functional writing style about writing a paper:\\
& & Write a passage with a flowery writing style about writing a paper:\\
\cmidrule(lr){2-3}
& \multirow{12}{*}{\textbf{Advanced}} & Write a candid passage about sunsets:\\
& & Write a prosaic passage about sunsets:\\
& & Write an ornate passage about sunsets:\\
& & Write a poetic passage about sunsets:\\
& & Write a candid passage about strawberries:\\
& & Write a prosaic passage about strawberries:\\
& & Write an ornate passage about strawberries:\\
& & Write a poetic passage about strawberries:\\
& & Write a candid passage about writing a paper:\\
& & Write a prosaic passage about writing a paper:\\
& & Write an ornate passage about writing a paper:\\
& & Write a poetic passage about writing a paper:\\
\midrule
\multirow{32}{*}{\textbf{Tone}} & \multirow{4}{*}{\textbf{Base}} & Write a dramatic passage about love:\\
& & Write a humorous passage about love:\\
& & Write an optimistic passage about love:\\
& & Write a sad passage about love:\\
\cmidrule(lr){2-3}
& \multirow{4}{*}{\textbf{Subject 2}} & Write a dramatic passage about life:\\
& & Write a humorous passage about life:\\
& & Write a optimistic passage about life:\\
& & Write a sad passage about life:\\
\cmidrule(lr){2-3}
& \multirow{4}{*}{\textbf{Subject 3}} & Write a dramatic passage about humanity:\\
& & Write a humorous passage about humanity:\\
& & Write a optimistic passage about humanity:\\
& & Write a sad passage about humanity:\\
\cmidrule(lr){2-3}
& \multirow{4}{*}{\textbf{Template 2}} & Write a passage about love with a dramatic tone:\\
& & Write a passage about love with a humorous tone:\\
& & Write a passage about love with an optimistic tone:\\
& & Write a passage about love with a sad tone:\\
\cmidrule(lr){2-3}
& \multirow{4}{*}{\textbf{Template 3}} & Create a dramatic passage about love:\\
& & Create a humorous passage about love:\\
& & Create an optimistic passage about love:\\
& & Create a sad passage about love:\\
\cmidrule(lr){2-3}
\pagebreak
& \multirow{8}{*}{\textbf{Advanced}} & Write an emotional passage about love:\\
& & Write a nostalgic passage about love:\\
& & Write an ironic passage about love:\\
& & Write a satirical passage about love:\\
& & Write an uplifting passage about love:\\
& & Write an inspirational passage about love:\\
& & Write a bleak passage about love:\\
& & Write a grim passage about love:\\
\cmidrule(lr){2-3}
& \multirow{4}{*}{\textbf{Useful}} & Write a formal passage about love:\\
& & Write an informal passage about love:\\
& & Write an assertive passage about love:\\
& & Write a passive-aggressive passage about love:\\
\midrule
\multirow{27}{*}{\textbf{Mood}} & \multirow{4}{*}{\textbf{Base}} & Write a passage about love that makes the reader feel angry:\\
& & Write a passage about love that makes the reader feel fearful:\\
& & Write a passage about love that makes the reader feel happy:\\
& & Write a passage about love that makes the reader feel sad:\\
\cmidrule(lr){2-3}
& \multirow{4}{*}{\textbf{Subject 2}} & Write a passage about life that makes the reader feel angry:\\
& & Write a passage about life that makes the reader feel fearful:\\
& & Write a passage about life that makes the reader feel happy:\\
& & Write a passage about life that makes the reader feel sad:\\
\cmidrule(lr){2-3}
& \multirow{4}{*}{\textbf{Subject 3}} & Write a passage about humanity that makes the reader feel angry:\\
& & Write a passage about humanity that makes the reader feel fearful:\\
& & Write a passage about humanity that makes the reader feel happy:\\
& & Write a passage about humanity that makes the reader feel sad:\\
\cmidrule(lr){2-3}
& \multirow{4}{*}{\textbf{Template 2}} & Write a passage about love with an angry mood:\\
& & Write a passage about love with a fearful mood:\\
& & Write a passage about love with a happy mood:\\
& & Write a passage about love with a sad mood:\\
\cmidrule(lr){2-3}
& \multirow{4}{*}{\textbf{Template 3}} & Create a passage about love that makes the reader feel angry:\\
& & Create a passage about love that makes the reader feel fearful:\\
& & Create a passage about love that makes the reader feel happy:\\
& & Create a passage about love that makes the reader feel sad:\\
\cmidrule(lr){2-3}
& \multirow{4}{*}{\textbf{Template 4}} &  Write a passage about love that makes the reader feel anger:\\
& & Write a passage about love that makes the reader feel fear:\\
& & Write a passage about love that makes the reader feel happiness:\\
& & Write a passage about love that makes the reader feel sadness:\\
\cmidrule(lr){2-3}
& \multirow{7}{*}{\textbf{Advanced}} & Write a passage about love that makes the reader feel envious:\\
& & Write a passage about love that makes the reader feel anxious:\\
& & Write a passage about love that makes the reader feel proud:\\
& & Write a passage about love that makes the reader feel regretful:\\
& & Write a passage about love that makes the reader feel surprised:\\
& & Write a passage about love that makes the reader feel loved:\\
& & Write a passage about love that makes the reader feel disgusted:\\
\midrule
\pagebreak
\multirow{10}{*}{\textbf{Characterization}} & \multirow{2}{*}{\textbf{Base}} & Write a story about lovers with indirect characterization:\\
& & Write a story about lovers with direct characterization:\\
\cmidrule(lr){2-3}
& \multirow{2}{*}{\textbf{Subject 2}}  & Write a story about cats with indirect characterization:\\
& & Write a story about cats with direct characterization:\\
\cmidrule(lr){2-3}
& \multirow{2}{*}{\textbf{Subject 3}}  & Write a story about survivors with indirect characterization:\\
& & Write a story about survivors with direct characterization:\\
\cmidrule(lr){2-3}
& \multirow{2}{*}{\textbf{Template 2}}  & Write a story about lovers where the characters are described directly:\\
& & Write a story about lovers where the characters are described indirectly:\\
\cmidrule(lr){2-3}
& \multirow{2}{*}{\textbf{Template 3}}  & Create a story about lovers with indirect characterization:\\
& & Create a story about lovers with direct characterization:\\
\midrule
\multirow{10}{*}{\textbf{Pacing}} & \multirow{2}{*}{\textbf{Base}} & Write a fast-paced story about lovers:\\
& & Write a slow-paced story about lovers:\\
\cmidrule(lr){2-3}
& \multirow{2}{*}{\textbf{Subject 2}} & Write a fast-paced story about cats:\\
& & Write a slow-paced story about cats:\\
\cmidrule(lr){2-3}
& \multirow{2}{*}{\textbf{Subject 3}} & Write a fast-paced story about survivors:\\
& & Write a slow-paced story about survivors:\\
\cmidrule(lr){2-3}
& \multirow{2}{*}{\textbf{Template 2}} & Write a story about lovers that is fast-paced:\\
& & Write a story about lovers that is slow-paced:\\
\cmidrule(lr){2-3}
& \multirow{2}{*}{\textbf{Template 3}} & Create a fast-paced story about lovers:\\
& & Create a slow-paced story about lovers:\\
\midrule
\multirow{35}{*}{\textbf{Plot}} & \multirow{7}{*}{\textbf{Base}} & Write a story about lovers with an "Overcoming the Monster" plot:\\
& & Write a story about lovers with a "Rags to Riches" plot:\\
& & Write a story about lovers with a "The Quest" plot:\\
& & Write a story about lovers with a "Voyage and Return" plot:\\
& & Write a story about lovers with a "Comedy" plot:\\
& & Write a story about lovers with a "Tragedy" plot:\\
& & Write a story about lovers with a "Rebirth" plot:\\
\cmidrule(lr){2-3}
& \multirow{7}{*}{\textbf{Subject 2}} & Write a story about cats with an "Overcoming the Monster" plot:\\
& & Write a story about cats with a "Rags to Riches" plot:\\
& & Write a story about cats with a "The Quest" plot:\\
& & Write a story about cats with a "Voyage and Return" plot:\\
& & Write a story about cats with a "Comedy" plot:\\
& & Write a story about cats with a "Tragedy" plot:\\
& & Write a story about cats with a "Rebirth" plot:\\
\cmidrule(lr){2-3}
& \multirow{7}{*}{\textbf{Subject 3}} & Write a story about survivors with an "Overcoming the Monster" plot:\\
& & Write a story about survivors with a "Rags to Riches" plot:\\
& & Write a story about survivors with a "The Quest" plot:\\
& & Write a story about survivors with a "Voyage and Return" plot:\\
& & Write a story about survivors with a "Comedy" plot:\\
& & Write a story about survivors with a "Tragedy" plot:\\
& & Write a story about survivors with a "Rebirth" plot:\\
\cmidrule(lr){2-3}
\pagebreak
& \multirow{7}{*}{\textbf{Subject 4}} & Write a story with an "Overcoming the Monster" plot:\\
& & Write a story with a "Rags to Riches" plot:\\
& & Write a story with a "The Quest" plot:\\
& & Write a story with a "Voyage and Return" plot:\\
& & Write a story with a "Comedy" plot:\\
& & Write a story with a "Tragedy" plot:\\
& & Write a story with a "Rebirth" plot:\\
\cmidrule(lr){2-3}
& \multirow{7}{*}{\textbf{Template 2}} & Create a story about lovers with an "Overcoming the Monster" plot:\\
& & Create a story about lovers with a "Rags to Riches" plot:\\
& & Create a story about lovers with a "The Quest" plot:\\
& & Create a story about lovers with a "Voyage and Return" plot:\\
& & Create a story about lovers with a "Comedy" plot:\\
& & Create a story about lovers with a "Tragedy" plot:\\
& & Create a story about lovers with a "Rebirth" plot:\\
\midrule
\multirow{36}{*}{\textbf{Genre}} & \multirow{6}{*}{\textbf{Base}} & Write a historical fiction story about lovers:\\
& & Write a literary fiction story about lovers:\\
& & Write a mystery story about lovers:\\
& & Write a science fiction story about lovers:\\
& & Write a dystopian story about lovers:\\
& & Write a horror story about lovers:\\
\cmidrule(lr){2-3}
& \multirow{6}{*}{\textbf{Subject 2}} & Write a historical fiction story about cats:\\
& & Write a literary fiction story about cats:\\
& & Write a mystery story about cats:\\
& & Write a science fiction story about cats:\\
& & Write a dystopian story about cats:\\
& & Write a horror story about cats:\\
\cmidrule(lr){2-3}
& \multirow{6}{*}{\textbf{Subject 3}} & Write a historical fiction story about survivors:\\
& & Write a literary fiction story about survivors:\\
& & Write a mystery story about survivors:\\
& & Write a science fiction story about survivors:\\
& & Write a dystopian story about survivors:\\
& & Write a horror story about survivors:\\
\cmidrule(lr){2-3}
& \multirow{6}{*}{\textbf{Subject 4}} & Write a historical fiction story:\\
& & Write a literary fiction story:\\
& & Write a mystery story:\\
& & Write a science fiction story:\\
& & Write a dystopian story:\\
& & Write a horror story:\\
\cmidrule(lr){2-3}
& \multirow{6}{*}{\textbf{Template 2}} & Write a story about lovers in a historical fiction genre:\\
& & Write a story about lovers in a literary fiction genre:\\
& & Write a story about lovers in a mystery genre:\\
& & Write a story about lovers in a science fiction genre:\\
& & Write a story about lovers in a dystopian genre:\\
& & Write a story about lovers in a horror genre:\\
\cmidrule(lr){2-3}
& \multirow{6}{*}{\textbf{Template 3}} & Create a historical fiction story about lovers:\\
& & Create a literary fiction story about lovers:\\
& & Create a mystery story about lovers:\\
& & Create a science fiction story about lovers:\\
& & Create a dystopian story about lovers:\\
& & Create a horror story about lovers:\\
\midrule
\multirow[c]{36}{*}{\textbf{Numerical}} & \multirow{27}{*}{\textbf{Base}}  & Write a sentence with five words about love:\\
& & Write a sentence with five words about cats:\\
& & Write a sentence with five words about running:\\
& & Write a sentence with ten words about love:\\
& & Write a sentence with ten words about cats:\\
& & Write a sentence with ten words about running:\\
& & Write a sentence with twenty words about love:\\
& & Write a sentence with twenty words about cats:\\
& & Write a sentence with twenty words about running:\\
& & Write a paragraph with five sentences about love:\\
& & Write a paragraph with five sentences about cats:\\
& & Write a paragraph with five sentences about running:\\
& & Write a paragraph with ten sentences about love:\\
& & Write a paragraph with ten sentences about cats:\\
& & Write a paragraph with ten sentences about running:\\
& & Write a paragraph with twenty sentences about love:\\
& & Write a paragraph with twenty sentences about cats:\\
& & Write a paragraph with twenty sentences about running:\\
& & Write a passage with five paragraphs about love:\\
& & Write a passage with five paragraphs about cats:\\
& & Write a passage with five paragraphs about running:\\
& & Write a passage with ten paragraphs about love:\\
& & Write a passage with ten paragraphs about cats:\\
& & Write a passage with ten paragraphs about running:\\
& & Write a passage with twenty paragraphs about love:\\
& & Write a passage with twenty paragraphs about cats:\\
& & Write a passage with twenty paragraphs about running:\\
\cmidrule(lr){2-3}
& \multirow{27}{*}{\textbf{Template 2}} & Write a sentence about love with 5 words:\\
& & Write a sentence about cats with 5 words:\\
& & Write a sentence about running with 5 words:\\
& & Write a sentence about love with 10 words:\\
& & Write a sentence about cats  with 10 words:\\
& & Write a sentence about running with 10 words:\\
& & Write a sentence about love with 20 words:\\
& & Write a sentence about cats with 20 words:\\
& & Write a sentence about running with 20 words:\\
& & Write a paragraph about love with 5 sentences:\\
& & Write a paragraph about cats with 5 sentences:\\
& & Write a paragraph about running with 5 sentences:\\
& & Write a paragraph about love  with 10 sentences:\\
& & Write a paragraph about cats with 10 sentences:\\
& & Write a paragraph about running with 10 sentences:\\
& & Write a paragraph about love with 20 sentences:\\
& & Write a paragraph about cats with 20 sentences:\\
& & Write a paragraph about running with 20 sentences:\\
& & Write a passage about love with 5 paragraphs:\\
& & Write a passage about cats with 5 paragraphs:\\
& & Write a passage about running with 5 paragraphs:\\
& & Write a passage about love with 10 paragraphs:\\
& & Write a passage about cats with 10 paragraphs:\\
& & Write a passage about running with 10 paragraphs:\\
& & Write a passage about love with 20 paragraphs:\\
& & Write a passage about cats  with 20 paragraphs:\\
& & Write a passage about running  with 20 paragraphs:\\
\midrule
\multirow{36}{*}{\textbf{Descriptive}} & \multirow{18}{*}{\textbf{Base}}  & Write a short passage about love:\\
& & Write a brief passage about love:\\
& & Write a concise passage about love:\\
& & Write a long passage about love:\\
& & Write a detailed passage about love:\\
& & Write an in-depth passage about love:\\
& & Write a short passage about cats:\\
& & Write a brief passage about cats:\\
& & Write a concise passage about cats:\\
& & Write a long passage about cats:\\
& & Write a detailed passage about cats:\\
& & Write an in-depth passage about cats:\\
& & Write a short passage about running:\\
& & Write a brief passage about running:\\
& & Write a concise passage about running:\\
& & Write a long passage about running:\\
& & Write a detailed passage about running:\\
& & Write an in-depth passage about running:\\
\cmidrule(lr){2-3}
& \multirow{18}{*}{\textbf{Template 2}} & Write a passage about love that is short:\\
& & Write a passage about love that is brief:\\
& & Write a passage about love that is concise:\\
& & Write a passage about love that is long:\\
& & Write a passage about love that is detailed:\\
& & Write a passage about love that is in-depth:\\
& & Write a passage about cats that is short:\\
& & Write a passage about cats that is brief:\\
& & Write a passage about cats that is concise:\\
& & Write a passage about cats that is long:\\
& & Write a passage about cats that is detailed:\\
& & Write a passage about cats that is in-depth:\\
& & Write a passage about running that is short:\\
& & Write a passage about running that is brief:\\
& & Write a passage about running that is concise:\\
& & Write a passage about running that is long:\\
& & Write a passage about running that is detailed:\\
& & Write a passage about running that is in-depth:\\
\midrule
\pagebreak
\multirow{36}{*}{\textbf{Functional}} & \multirow{8}{*}{\textbf{Code}}  & Code Python code that plays the game of war:\\
& & Code Python code that sums two integers up:\\
& & Code C code that plays the game of war:\\
& & Code C code that sums two integers up:\\
& & Write Python code that plays the game of war:\\
& & Write Python code that sums two integers up:\\
& & Write C code that plays the game of war:\\
& & Write C code that sums two integers up:\\
\cmidrule(lr){2-3}
& \multirow{6}{*}{\textbf{Email}} & Write an email to my teacher:\\
& & Write an email to my teacher asking for help on math homework:\\
& & Write an email to my boyfriend:\\
& & Write an email to my boyfriend to arrange a date this Saturday:\\
& & Write an email to my client:\\
& & Write an email to my client requesting a copy of the updated contract:\\
\cmidrule(lr){2-3}
& \multirow{10}{*}{\textbf{Academic Paper}} & Write a properly formatted academic paper on artificial intelligence:\\
& & Write an academic paper on artificial intelligence in the proper format:\\
& & Write a properly formatted academic paper on the flaws of GPT-3:\\
& & Write an academic paper on the flaws of GPT-3 in the proper format:\\
& & Write a properly formatted academic paper on strategies our society can adopt to recover after the global pandemic as quickly and painlessly as possible:\\
& & Write an academic paper on strategies our society can adopt to recover after the global pandemic as quickly and painlessly as possible in the proper format:\\
\bottomrule
\caption{The full list of the prompts.}
\label{tab:prompts}
\end{longtable}

\begin{table*}[h]
\scalebox{1}{
    \begin{tabular}{@{}cl@{}}
    \toprule
    
    0 & Write a flowery passage about sunsets:\\
    1 & Write a humorous passage about love:\\
    2 & Write a passage about love that makes the reader feel fearful:\\
    3 & Write a story about lovers with indirect characterization:\\
    4 & Write a fast-paced story about lovers:\\
    5 & Write a story about lovers with a "Tragedy" plot:\\
    6 & Write a historical fiction story about lovers:\\
    \bottomrule
    \end{tabular}
}
\caption{\textbf{Selected prompts for additional experiments}}
\label{tab:selected_prompts}
\end{table*}



\clearpage
\twocolumn

==> 2022 ARR Limitations of LLM/Table/story.tex <==
\begin{table*}[t]
\centering
\resizebox{2\columnwidth}{!}{%
    \begin{tabular}{@{}llccccccc@{}}
    \toprule
    \multirow{2}{*}{\textbf{Aspect}} & \multirow{2}{*}{\textbf{Category}} &
    \multirow{2}{*}{\textbf{Base}} & \multicolumn{2}{c}{\textbf{Template}} &
    \multicolumn{3}{c}{\textbf{Subject}} &
    \multirow{2}{*}{\textbf{Mean}}\\ 
    \cmidrule(lr){4-5} \cmidrule(lr){6-8}
    & & & \textbf{2} & \textbf{3} & \textbf{Cats} & \textbf{Survivors} & \textbf{None}\\
    \midrule
    \multirow{2}{*}{Characterization}
    & Direct & 1.0\textsubscript{$\pm$0.54} & 0.77\textsubscript{$\pm$0.87} & 0.33\textsubscript{$\pm$0.77} & 0.53\textsubscript{$\pm$0.65} & 0.5\textsubscript{$\pm$0.82} & / & 0.63 \\
    & Indirect & 0.7\textsubscript{$\pm$0.64} & 0.93\textsubscript{$\pm$0.42} & 0.77\textsubscript{$\pm$0.37} & 0.87\textsubscript{$\pm$0.58} & 0.1\textsubscript{$\pm$0.72} & / & 0.67\\
    \midrule
    \multirow{2}{*}{Pacing}
    & Fast & 1.23\textsubscript{$\pm$0.72} & 0.77\textsubscript{$\pm$0.7} & 1.3\textsubscript{$\pm$0.31} & 1.03\textsubscript{$\pm$0.6} & 0.9\textsubscript{$\pm$0.58} & / & 1.05\\
    & Slow & 0.53\textsubscript{$\pm$0.88} & 0.7\textsubscript{$\pm$0.55} & 0.97\textsubscript{$\pm$0.62} & 0.73\textsubscript{$\pm$0.76} & 0.67\textsubscript{$\pm$0.67} & / & 0.72\\
    \midrule
    \multirow{7}{*}{Plot}
    & Overcoming the Monster & 0.37\textsubscript{$\pm$0.91} & 1.0\textsubscript{$\pm$0.75} & / & 0.7\textsubscript{$\pm$0.94} & 1.33\textsubscript{$\pm$0.3} & 1.53\textsubscript{$\pm$0.31} & 0.99 \\
    & Rags to Riches & 1.33\textsubscript{$\pm$0.71} & 0.77\textsubscript{$\pm$0.87} & / & 0.5\textsubscript{$\pm$0.85} & 0.27\textsubscript{$\pm$0.9} & 1.53\textsubscript{$\pm$0.65} & 0.88\\
    & The Quest & 1.33\textsubscript{$\pm$0.54} & 1.2\textsubscript{$\pm$0.48} & / & 1.37\textsubscript{$\pm$0.38} & 1.27\textsubscript{$\pm$0.39} & 1.6\textsubscript{$\pm$0.25} & 1.35\\
    & Voyage and Return & 1.07\textsubscript{$\pm$0.53} & 1.27\textsubscript{$\pm$0.42} & / & 1.33\textsubscript{$\pm$0.54} & 1.1\textsubscript{$\pm$0.54} & 1.3\textsubscript{$\pm$0.28} & 1.21\\
    & Comedy & -0.3\textsubscript{$\pm$0.9} & -0.3\textsubscript{$\pm$0.84} & / & -0.07\textsubscript{$\pm$0.99} & -0.5\textsubscript{$\pm$0.48} & 0.03\textsubscript{$\pm$0.85} & -0.23\\
    & Tragedy & 1.6\textsubscript{$\pm$0.39} & 1.8\textsubscript{$\pm$0.27} & / & 1.27\textsubscript{$\pm$0.59} & 0.63\textsubscript{$\pm$0.38} & 1.5\textsubscript{$\pm$0.4} & 1.36\\
    & Rebirth & 1.13\textsubscript{$\pm$0.56} & 1.33\textsubscript{$\pm$0.65} & / & 0.93\textsubscript{$\pm$0.81} & 1.03\textsubscript{$\pm$0.55} & 1.4\textsubscript{$\pm$0.39} & 1.16\\
    \midrule
    \multirow{6}{*}{Genre}
    & Historical fiction & 0.77\textsubscript{$\pm$0.93} & 1.07\textsubscript{$\pm$1.08} & 0.97\textsubscript{$\pm$0.72} & -0.2\textsubscript{$\pm$0.93} & 0.43\textsubscript{$\pm$0.92} & 1.13\textsubscript{$\pm$0.99} & 0.70\\
    & Literary fiction & 0.87\textsubscript{$\pm$0.65} & 0.8\textsubscript{$\pm$0.48} & 0.97\textsubscript{$\pm$0.57} & 0.4\textsubscript{$\pm$0.84} & 0.9\textsubscript{$\pm$0.6} & 0.27\textsubscript{$\pm$0.42} & 0.70\\
    & Science fiction & 0.47\textsubscript{$\pm$0.76} & 0.9\textsubscript{$\pm$0.82} & 0.37\textsubscript{$\pm$0.84} & 1.5\textsubscript{$\pm$0.31} & 1.13\textsubscript{$\pm$0.5} & 1.47\textsubscript{$\pm$0.52} & 0.97\\
    & Mystery & 1.1\textsubscript{$\pm$0.58} & 1.6\textsubscript{$\pm$0.39} & 1.23\textsubscript{$\pm$0.45} & 1.4\textsubscript{$\pm$0.36} & 0.73\textsubscript{$\pm$0.9} & 1.67\textsubscript{$\pm$0.45} & 1.29\\
    & Dystopian & 1.37\textsubscript{$\pm$0.43} & 1.63\textsubscript{$\pm$0.43} & 1.5\textsubscript{$\pm$0.45} & 1.53\textsubscript{$\pm$0.56} & 1.6\textsubscript{$\pm$0.33} & 1.8\textsubscript{$\pm$0.31} & 1.57\\
    & Horror & 1.23\textsubscript{$\pm$0.67} & 1.07\textsubscript{$\pm$0.93} & 1.63\textsubscript{$\pm$0.28} & 1.4\textsubscript{$\pm$0.74} & 1.57\textsubscript{$\pm$0.65} & 1.47\textsubscript{$\pm$0.62} & 1.40\\
    \bottomrule
    \end{tabular}
}
\caption{\textbf{Results for story-centric stylistic constraints}. All but subject variations use the subject "lovers".
%All but template variations use template 1. We show the full prompt lists in Appendix~\ref{app:prompt_list}.
}
%What is template 1?
\label{tab:story}
\end{table*}

==> 2022 ARR Limitations of LLM/Table/summary.tex <==
\begin{table}[t]
\centering
\scalebox{0.78}{
    \begin{tabular}{@{}llll@{}}
    \toprule
    \textbf{Aspect} & \textbf{Example Terms} & \textbf{Fail} \\
    \midrule
    Writing Style & Flowery, Functional & Sometimes\\
    Tone & Humorous, Formal & Occasionally\\
    Mood & Angry, Sad & Sometimes\\
    Characterization & Direct, Indirect & Often \\
    Pacing & Fast, Slow & Often\\
    Plot & Rebirth, Comedy, & Occasionally\\
    Genre & Science Fiction, Mystery & Sometimes\\
    \midrule
    Numerical & Five words, Ten sentences & Often\\
    Descriptive & Concise, Long & Occasionally\\
    Formatting & Email, Code & Occasionally\\
    \bottomrule
    \end{tabular}
}
\caption{\textbf{Summary of our taxonomy and results}. We show the full list of prompts in Appendix~\ref{app:prompt_list}.}
\label{tab:summary}
\end{table}

% \begin{table*}[t]
% \scalebox{1}{
%     \begin{tabular}{@{}llll@{}}
%     \toprule
%     \textbf{Aspect} & \textbf{Terms} & \textbf{Example Prompt} & \textbf{Fail} \\
%     \midrule
%     Numerical & Five, Ten, Twenty & \textit{Write a sentence with \textbf{five words} about love} & Often\\
%     Granularity & Short, Concise, Long, Detailed & \textit{Write a \textbf{short} passage about love} & Occasionally\\
%     Functional & & \textit{Write an \textbf{email} to my teacher} & Occasionally\\
%     \midrule
%     Writing Style & & \textit{Write a \textbf{flowery} passage about sunsets} & Sometimes\\
%     Tone & & \textit{Write a \textbf{humorous} passage about love} & Occasionally\\
%     Mood & & \textit{Write a passage about love that makes the reader feel \textbf{fearful}} & Sometimes\\
%     Characterization & & \textit{Write a story about lovers with \textbf{indirect} characterization} & Often \\
%     Pacing & & \textit{Write a \textbf{fast-paced} story about lovers} & Often\\
%     Plot & & \textit{Write a story about lovers with a \textbf{"Tragedy"} plot} & Occasionally\\
%     Genre & & \textit{Write a \textbf{historical fiction} story about lovers} & Sometimes\\
%     \bottomrule
%     \end{tabular}
% }
% \caption{\textbf{Summary of our taxonomy and results}. We show the full prompt lists in Appendix~\ref{app:prompt_list}.}
% \label{tab:summary}
% \end{table*}

==> 2022 ARR Limitations of LLM/Table/tone_mood.tex <==
\begin{table*}[t]
\scalebox{1}{
    \begin{tabular}{@{}llccccccc@{}}
    \toprule
    \multirow{2}{*}{\textbf{Aspect}} & \multirow{2}{*}{\textbf{Category}} &
    \multirow{2}{*}{\textbf{Base}} & \multicolumn{3}{c}{\textbf{Template}} &
    \multicolumn{2}{c}{\textbf{Subject}} &
    \multirow{2}{*}{\textbf{\underline{Mean}}}\\ 
    \cmidrule(lr){4-6} \cmidrule(lr){7-8}
    & & & \textbf{2} & \textbf{3} & \textbf{4} & \textbf{Life} & \textbf{Humanity} & \\
    \midrule
    \multirow{4}{*}{Tone} & Dramatic & 1.1\textsubscript{$\pm$0.7} & 1.43\textsubscript{$\pm$0.5} & 1.37\textsubscript{$\pm$0.28} & / & 1.37\textsubscript{$\pm$0.38} & 1.5\textsubscript{$\pm$0.22} & 1.35\\
    & Humorous & -0.5\textsubscript{$\pm$0.48} & -0.2\textsubscript{$\pm$0.6} & 0.3\textsubscript{$\pm$1.17} & / & -0.1\textsubscript{$\pm$0.9} & -0.03\textsubscript{$\pm$0.92} & -0.11\\
    & Optimistic & 1.3\textsubscript{$\pm$0.43} & 1.63\textsubscript{$\pm$0.48} & 1.6\textsubscript{$\pm$0.36} & / & 1.7\textsubscript{$\pm$0.23} & 1.67\textsubscript{$\pm$0.26} & 1.58\\
    & Sad & 1.27\textsubscript{$\pm$0.36} & 1.03\textsubscript{$\pm$0.64} & 1.17\textsubscript{$\pm$0.6} & / & 1.5\textsubscript{$\pm$0.4} & 1.17\textsubscript{$\pm$0.48} & 1.23 \\
    \midrule
    \multirow{4}{*}{Mood} & Angry & 0.37\textsubscript{$\pm$0.41} & 0.93\textsubscript{$\pm$0.8} & 0.2\textsubscript{$\pm$0.9} & 0.83\textsubscript{$\pm$0.89} & 0.8\textsubscript{$\pm$0.96} & 1.2\textsubscript{$\pm$0.62} & 0.72\\
    & Fearful & 0.57\textsubscript{$\pm$0.7} & 0.77\textsubscript{$\pm$0.54} & 0.77\textsubscript{$\pm$0.52} & 0.67\textsubscript{$\pm$0.86} & 1.4\textsubscript{$\pm$0.42} & 1.33\textsubscript{$\pm$0.3} & 0.92\\
    & Happy & 1.57\textsubscript{$\pm$0.26} & 1.3\textsubscript{$\pm$0.28} & 1.4\textsubscript{$\pm$0.33} & 1.37\textsubscript{$\pm$0.31} & 1.47\textsubscript{$\pm$0.31} & 1.33\textsubscript{$\pm$0.54} & 1.41\\
    & Sad & 1.27\textsubscript{$\pm$0.59} & 1.3\textsubscript{$\pm$0.46} & 1.03\textsubscript{$\pm$0.46} & 0.9\textsubscript{$\pm$0.68} & 1.33\textsubscript{$\pm$0.49} & 0.9\textsubscript{$\pm$0.58} & 1.12 \\
    \bottomrule
    \end{tabular}
}
\caption{\textbf{Results for basic tones and moods}. All but subject variations use subject ``love''. %All but template variations use template 1. We show the full prompt lists in Appendix~\ref{app:prompt_list}.
}
\label{tab:tone_mood_basic}
\end{table*}

==> 2022 ARR Limitations of LLM/Table/writing_style.tex <==
\begin{table}[t]
\centering
\scalebox{0.78}{
    \begin{tabular}{@{}lccc@{}}
    \toprule
    \multirow{2}{*}{\textbf{Writing Style}} & \multicolumn{3}{c}{\textbf{Subject}} \\ 
    \cmidrule(lr){2-4} & \textbf{Sunsets} & \textbf{Strawberries} & \textbf{Writing a paper} \\
    \midrule
    \multirow{2}{*}{\textbf{Functional}} & 0.27\textsubscript{$\pm$0.66} & 1.47\textsubscript{$\pm$0.31} & 1.67\textsubscript{$\pm$0.26} \\
     & 0.40\textsubscript{$\pm$0.83} & 1.50\textsubscript{$\pm$0.43} & 1.53\textsubscript{$\pm$0.48} \\
     \midrule
    \multirow{2}{*}{\textbf{Flowery}} & 1.03\textsubscript{$\pm$0.77} & 0.63\textsubscript{$\pm$1.00} & 1.03\textsubscript{$\pm$0.48} \\
     & 1.27\textsubscript{$\pm$0.44} & 0.97\textsubscript{$\pm$0.77} & -0.13\textsubscript{$\pm$0.92} \\
    \midrule
    \textbf{Candid} & 1.20\textsubscript{$\pm$0.56} & 1.27\textsubscript{$\pm$0.25} & 1.50\textsubscript{$\pm$0.27} \\
    \textbf{Prosaic} & 0.07\textsubscript{$\pm$0.92} & 1.03\textsubscript{$\pm$0.66} & 1.23\textsubscript{$\pm$0.78} \\
    \textbf{Ornate} & 1.17\textsubscript{$\pm$0.54} & 0.67\textsubscript{$\pm$1.04} & 0.83\textsubscript{$\pm$0.45} \\
    \textbf{Poetic} & 1.77\textsubscript{$\pm$0.40} & 1.10\textsubscript{$\pm$0.83} & 1.33\textsubscript{$\pm$0.47} \\\bottomrule
    \end{tabular}
}
\caption{\textbf{Results for Writing Style}. The average of the annotation score (with standard error) is reported (each score is in the range of (-2, 2)). Each row of \textbf{Functional} and \textbf{Flowery} represents a different prompt template (Semantically identical but syntactically different prompt).}
\label{tab:wrting_style}
\end{table}

==> Table/BLOOM.tex <==
\begin{table*}[ht]{
    \begin{tabular}{p{\textwidth}}
        \toprule
        \textbf{Write a flowery passage about sunsets:} the setting sun, the west, the rising sun, and the east. Include in your writing the following words of imagery: ”flaming,” “melted,” “burnt,” “reddened,” and “blazing.”In the 1990s when I was a young man, I was heavily involved in the Fellowship of Reconciliation and its Quaker Peace and Social Justice campaigns. I was also a member of the Socialist Workers Party and the British Socialist Party. In 2003 I was elected a member of the Socialist Party’s national committee, and subsequently ran for parliamentary election as their candidate in the Kensington constituency in south west London, where I came third with 3.5\% of the vote. I am now a member of the Socialist Party and Socialist Workers Party.
         
As I have already said, I am proud to have been in the Socialist Workers Party from a very early age and to have been part of the SWP’s national executive committee from 2003 to 2009 and to have now been re-elected to its national committee. I am proud that the SWP remains a revolutionary Marxist party in Britain today.

I am not a member of the Labour Party. I have no interest in the Labour Party.\\
        \midrule
        \textbf{Write a humorous passage about love:}
         
Write a humorous passage about love:

Write a humorous passage about love:

Write a humorous passage about love:

Write a humorous passage about love:

Write a humorous passage about love:

Write a humorous passage about love:

Write a humorous passage about love:

Write a humorous passage about love:

Write a humorous passage about love:

Write a humorous passage about love:

Write a humorous passage about love:

Write a humorous passage about love:

Write a humorous passage about love:

Write a humorous passage about love:

Write a humorous passage about love:

Write a humorous passage about love:

Write a humorous passage about love:

Write a humorous passage about love:

Write a humorous passage about love:

Write a humorous passage about love:

Write a humorous passage about love:

Write a humorous passage about love:

Write a humorous passage about love:

Write a humorous passage about\\
        \midrule
        \textbf{Write a passage about love that makes the reader feel fearful:} The author’s goal is to tell a story, but instead of telling it in their own words, they use the words of others. The author’s goal is to tell a story, but instead of telling it in their own words, they use the words of others. The author’s goal is to tell a story, but instead of telling it in their own words, they use the words of others. The author’s goal is to tell a story, but instead of telling it in their own words, they use the words of others. The author’s goal is to tell a story, but instead of telling it in their own words, they use the words of others. The author’s goal is to tell a story, but instead of telling it in their own words, they use the words of others. The author’s goal is to tell a story, but instead of telling it in their own words, they use the words of others. The author’s goal is to tell a story, but instead of telling it in their own words, they use the words of others. The author’s goal is to tell a story, but instead of telling it in their own words, they use the words of others. The author’s goal is to tell\\
        \bottomrule
    \end{tabular}
}
\caption{Responses from BLOOM-176B.}
\end{table*}

==> Table/Mitigations_and_Models.tex <==
\begin{table}[t]
\centering
\scalebox{0.94}{
    \begin{tabular}{@{}lcc@{}}
    \toprule
    \textbf{LLM} & \textbf{Mean Score} \\
    \midrule
    GPT-3 A & 0\% & 0.77\\
    GPT-3 B & 53\% & -0.94\\
    GPT-3 C & 71\% & -1.41\\
    GPT-3 D, t = 0.4 & 
    GPT-3 D, t = 0.7 & 
    GPT-3 D, t = 1.0 & 57\% & -1.01 \\
    GPT-3 D
    \bottomrule
    \end{tabular}
}
\caption{Results on a trial experiment with 7 prompts from Table~\ref{tab:selected_prompts}. t = temperature}
\label{tab:mitigations_and_models}
\end{table}

==> Table/Style_result.tex <==
\begin{table}[t]
\scalebox{1}{
    \begin{tabular}{@{}llc@{}}
    \toprule
    \textbf{Aspect} & \textbf{Category} &
    \textbf{\underline{Score}}\\ 
    \midrule
    \multirow{4}{*}{Tone} & Dramatic & 1.35\\
    & Humorous & -0.11\\
    & Optimistic & 1.58\\
    & Sad & 1.23 \\
    \midrule
    \multirow{4}{*}{Mood} & Angry & 0.72\\
    & Fearful & 0.92\\
    & Happy & 1.41\\
    & Sad & 1.12 \\
    \bottomrule
    \end{tabular}
}
\caption{\textbf{Main results for stylistic constraints}. The score reported here is averaged over all prompt templates and subjects. We show the detailed result for each template and subject in Appendix~\ref{app:additional}.
}
\label{tab:style_result}
\end{table}
